Graph Sparsification for GCN Towards Optimal Crop Yield Predictions

In agronomics, predicting crop yield at a per field/county granularity is important for farmers to minimize uncertainty and plan seeding for the next crop cycle. While state-of-the-art prediction techniques employ graph convolutional nets (GCN) to predict future crop yields given relevant features and crop yields of previous years, a dense underlying graph kernel requires long training and execution time. In this paper, we propose a graph sparsification method based on the Fiedler number to remove edges from a complete graph kernel, in order to lower the complexity of GCN training/execution. Specifically, we first show that greedily removing an edge at a time that induces the minimal change in the second eigenvalue leads to a sparse graph with good GCN performance. We then propose a fast method to choose an edge for removal per iteration based on an eigenvalue perturbation theorem. Experiments show that our Fiedler-based method produces a sparse graph with good GCN performance compared to other graph sparsification schemes in crop yield prediction.

==> Methodology.tex <==
%We assume a slowly time-varying dynamic graph model, where the optimal graph Laplacian $\L_t$ at time $t$ differs from $\L_{t+1}$ at time $t+1$ differs by a low-rank matrix $\G$. 

%\begin{align}
%\min_{\G,\N} &~ \|\O - \L_{t+1}\|_F + \|\G\|_* + \|\N\|_F \\
%&\mbox{s.t.}~~ \L_{t+1} = \L_t + \G + \N
%\end{align}
